DreamDistribution: Learning Prompt Distribution for Diverse In-distribution Generation

The popularization of Text-to-Image (T2I) diffusion models enables the generation of high-quality images from text descriptions. However, generating diverse customized images with reference visual attributes remains challenging. This work focuses on personalizing T2I diffusion models at a more abstract concept or category level, adapting commonalities from a set of reference images while creating new instances with sufficient variations. We introduce a solution that allows a pretrained T2I diffusion model to learn a set of soft prompts, enabling the generation of novel images by sampling prompts from the learned distribution. These prompts offer text-guided editing capabilities and additional flexibility in controlling variation and mixing between multiple distributions. We also show the adaptability of the learned prompt distribution to other tasks, such as text-to-3D. Finally we demonstrate effectiveness of our approach through quantitative analysis including automatic evaluation and human assessment. Project website: https://briannlongzhao.github.io/DreamDistribution

==> sections/0_teaser_cvpr.tex <==
% Teaser image
\twocolumn[{
% \renewcommand\twocolumn[1][]{#1}
\maketitle
\begin{center}
\vspace{-5pt}
    \centering
    \captionsetup{type=figure}
    \includegraphics[width=\textwidth]{figures/teaser\_7.png}
    \captionof{figure}{
        \method learns a prompt distribution $D^*$ that represents a distribution of descriptions corresponding to a set of reference images. We can sample new prompts from $D^*$ or modified $D^*$ by text-guided editing to generate images of diverse new instance that follows the visual attributes of reference training images (top). We can also apply a learned distribution flexibly to, for example, a pretrained text-to-3D model, and generate diverse new 3D assets following the reference images (bottom).
    }
    \label{fig:teaser}
\end{center}
}]



% \makeatletter
% \let\@oldmaketitle\@maketitle% Store \@maketitle
% \renewcommand{\@maketitle}{\@oldmaketitle% Update \@maketitle to insert...
%   \includegraphics[width=\linewidth,height=4\baselineskip]
%     {figures/teaser\_7.png}\bigskip}% ... an image
% \makeatother



==> sections/1_introduction.tex <==
\section{Introduction}
\label{sec:introduction}





Story outline:
\begin{itemize}
    \item Introduce T2I diffusion, typical T2I diffusion fine-tuning approach: prepare image data with caption
    \item{Typical scenarios of personalizing T2I model via finetuning: adapt multiple new concepts/styles, e.g., associate words of animals to pokemons, then need to prepare for example images of pikachu captioned by mouse, images of squirtle captioned by turtle, etc. Also personalizing for a debiased model, e.g. pretrained model generates only female for housekeeper, only red-colored firetrucks, etc, but we want to debias/diversify generated images.}
    \item Challenge 1: usually hard to prepare large scale image-caption pairs for specific needs
    \item Challenge 2: Also not able to provide detailed accurate text description for an image
    \item Therefore introduce prompt learning applied on T2I diffusion
    \item Challenge of using prompt learning: However it does not make sense to use a single prompt to describe all training images
    \item Therefore we propose learning a distribution for a set of images, and sample prompt from learnt prompt distribution for generation.
    \item By applying prompt distribution leaning, we are able to capture the distribution of features in training images, and generate new images not present in training set, but still follows the distribution of training set.
    \item In previous work, textual inversion learns a fix token embedding $S_*$ to represent a specific object instance, or a specific style/background.
    \item A single token embedding maybe not enough to encode a diverse set of images
    \item We instead learn $S_*^+$, a distribution of a sequence of token embeddings, that represents a prompt distribution corresponding to the input training images
    \item in experiment, we first show we can capture distribution of a diverse set of few training images (same category different instances) by learning a distribution of prompts ($S_*^+$)
    \item Compared to fix prompt, which might generate an average/combination of training images, prompt distribution should be able to generate more diverse images following training image distribution.
    \item We also show that we can transfer distribution of image styles when the training images is of different variation of styles i.e., different cartoons.
    \item We also apply our methods for synthetic data generation, where  foreground, background, everything is entangled in the images, prompt distribution learning can capture the distribution of images as a whole.
    \item Compare to previous works that use class names and manually designed prompts to generate training set, using our generated training set shows significant improvement of ImageNet classification accuracy on real validation set.
    \item We also show our learned prompt distribution can be applied to any downstream generation tasks that takes text as generation condition, e.g., 3D generation
    \item Applied on zero1to3 or mvdream, we can generate diverse 3D object assets that follows the general features of given some sample images.
    \item This might be useful for creating diverse 3D assets in game development that follows a specific artistic style/design.
\end{itemize}


\VV{Story 2:

Goal. Our goal is to personalize a text to image generation model to generate diverse images corresponding to multiple instances of a category by learning concepts from a small set of images describing those instances.


\begin{itemize}

\item Instance specific concept learning. Personalization of T2I model. Prior work like textual inversion learns relevant personalization concepts from images for any specific object instance level. Generates only instance specific images.

\item Category specific concept learning. Our focus is on personalizing T2I model at category level. A category may contain multiple object instances. Instances may differ in their appearance and physical properties. Examples: Teapot may come in different appearance and shapes. Transformer toys may come in different shapes and appearances. A personalized T2I model for a category should be able to learn concepts from different object instances and be able to generate such diverse images spanning across different object instances.

\item Applications and use scenario. 1) Training data generation. An object can come in different shapes, appearances, and in different context etc. Such information can be provided by a small number of images. Our approach can then use these images to generate new synthetic images spanning across different properties. 2) Personalizing T2I models from multiple instances. Learn concepts from multiple instances and then generate images corresponding these instances. 3) Personalizing T23D models from multiple instances.
\end{itemize}

}



\brian{
Story 3:
\begin{itemize}
    \item Introduce T2I diffusion, typical T2I diffusion fine-tuning approach: prepare image data with caption \VV{The question is why do we need to prepare image data with caption? Do we want to provide some motivation scenario to support why we need to prepare image data with caption. Like in training of a model.} 
    \VV{What is the accuracy on ImageNet? Are we able to get better than real data?}\brian{It seems impossible to get better result than real imagenet using only synthetic images, but we are better than other baselines, and mixing real and synthetic also gives significant improvement}
    \item Challenge 1: usually hard to prepare large scale image-caption pairs for specific needs
    \item Challenge 2: Also not able to provide detailed accurate text description for an image
    \item Therefore introduce prompt learning applied on T2I diffusion
    \item We show by experiment that using a fixed manually designed text prompts for each images of a small set, the generated images are not good, both visually and quantitatively (means and variances of train and generated not similar).
    \item Also using a fixed learnable prompt, the result also not satisfactory.
    \item Here we naturally introduce prompt distribution learning, and show results better than text prompt and fixed prompt learning
    \item Application scenario: same as above, personalize a category of objects, a set of style/texture, 3d object, and training data generation
    \VV{Are the story 3 and story 1 not the same?}
\end{itemize}
}



TODOs:
\begin{itemize}
    \item week 10/9: Try MVDream, Research on metrics, account for diversity, more experiments on refined distribution learning
    \item week 10/16: more experiments on refined distribution learning
\end{itemize}



Text-to-image (T2I) generation has recently been popularized due to the astonishing performance of state-of-the-art diffusion models such as Stable Diffusion \cite{rombach2021highresolution} and DALL·E 2 \cite{ramesh2022hierarchical}.
%
Beyond the simple text prompt to image generation approach, many variational pipelines enabled diffusion models to perform a variety of fascinating tasks, such as inpainting \cite{lugmayr2022repaint, Xie_2023_CVPR} and conditioned generation based on input of other modalities \cite{zhang2023adding, li2023gligen}.
%
Typically, when fine-tuning a T2I diffusion model, one needs to prepare a dataset consists of image-text pairs, where the text is a natural language description of the corresponding image. In many cases, however, a simple text description is not enough to describe the information of an image. 
%
This is the dilemma where users have to continuously try many different text prompts via a cumbersome prompt engineering process to get the desirable generated images.




On the other hand, prompt learning is a popular method of fine-tuning NLP models for specific downstream tasks. 
%
Instead of giving a natural language text as prompt, a sequence of learnable embeddings serve as the prompt input of language models, and therefore improve the model performance and reduce the number of training parameter in the model itself at the same time. 
%
This method is also proven to be useful when adapted to computer vision tasks and vision-language tasks as well \cite{jia2022visual, zhou2022learning}.



In this work, we propose to adapt prompt learning approach on T2I diffusion models.
%
Specifically, when fine-tuning the diffusion model using image-text paired data, instead of using fixed text prompt and updating the weights in diffusion model itself, we insert a sequence of learnable embeddings, concatenated with the embeddings of any other meaningful words, such as the class name or object description of a set of images, as the conditioning input. 
%
These learned embeddings can be treated as a set of learned descriptions of the training images. 
%
Although they might not interpretable by human as they lie in a continuous space, the pretrained T2I diffusion model should have the ability to understand the learned embedding and generate desirable outputs.
%
Additionally, we propose a modified approach to learn a distribution of prompt instead of a fixed prompt for a set of images. This prompt distribution should be able to capture a common characteristics of the images within the same set, e.g, style, texture, pose, etc.
%
More specifically, this could be done by keeping a collection of prompts corresponding to a same set of images, and the prompts could be orthogonal updated so that a normal distribution could be used to model the differently updated prompts.
%
During inference, we can then sample from the prompt distribution, which should have a similar "meaning", understood by the downstream diffusion model, to produce in-distribution but at the same time diverse outputs.



The learned prompts or distributions of prompts can be thus easily adopted to other T2I tasks. 
%
One of the straightforward use cases would be customized image generation.
%
By taking several images of an object of interest as training images, we can learn a fixed prompt to generate images of similar object, or by incorporating prompt distribution learning, we can generate a more diverse set of images. 
%
Another useful case might be synthetic data generation, where we use a small dataset to learn the prompts using T2I diffusion model and then generate a larger scale in-domain dataset with enough fidelity and diversity.
%
More broadly, learned prompts can be adapted to any other existing diffusion-based pipelines that take text as an conditioning input.
%
For example, using learned prompts for inpainting would allow model to in-paint the masked area with a customized object, and using learned prompts for text-to-3D generation would make it easy to generate different customized 3D objects of same style, etc.


==> sections/1_introduction_2.tex <==
\section{Introduction}
\label{sec:introduction}


\begin{itemize}

\item Personalization of T2I model. Finetuning, Textual inversion. They use images corresponding to object instances. \newline


Text to image synthesis models have achieved remarkable progress. They are able to generate really high quality images. Models like DALL-E, stable diffusion, etc. have achieved photo realism. More recent years, there has been efforts on personalizing these models to user specific requirements. Knowledge about personalization can be provided by a set of images corresponding the object of interest. This personalization of T2I models can be performed using fine-tuning. However, this can lead to catastrophic forgetting. Personalization using textual inversion has been an important approach for personalization using a set of images. It can generate really nice images. 

\item Issues. Only for instances. In general if we take random set of images for any object, there may be diversity in images. Another multiple instances for each object. \newline

Though these prior models can generate really high resolution images, they have some issues. First, training of these models mostly require images for object instances. So, there are no diversity in generated images. Second, any noise or variations in images corresponding to the object instance leads to noisy outputs. Third, in many real world applications, there is need to personalize T2I model at category level that can have multiple object instances. These instances can vary in shape and appearances. For instance, personalizing and generating images for transformer toys. 
%
The existing personalization T2I models cannot scale to these scenario where training images contain variations even if they come from same object instances or if they come from multiple instances. This leads to noisy outputs or no diversity in the generated images.

\item A desired properties of a method for personalization. \newline

In order to adapt/personalize a model to a user's requirement, any such personalization methods should have these properties. First, it should be able to be able to train using a random set of images corresponding to object instances. Furthermore, it should be able to be train using images from multiple object instances. Second, these models should learn concepts from these diverse sets of images and generate diverse images corresponding to the multiple objects. Finally, personalization should not lead to catastrophic forgetting of the original text to image diffusion model.

\item Proposed approach. \newline

In this paper, we propose a method for personalizing T2I generation model that can learn from a random set of training images corresponding to one or multiple object instances for a category. Second, it does not lead to any catatrophic forgetting. We do prompt optimization ... fill this part.

\item Applications.

We demonstrate the effectiveness of the proposed approach on several applications. First we demonstrate results of our approach in generating diverse set of personalized images and demonstrate benefits over prior approaches like textual inversion. Further, we extend our approach to 3D domain and show that our approach can effectively generate diverse set of 3D shapes. Finally, we use our approach to generate large scale images for training ImageNet data. Expand this.

\end{itemize}


==> sections/1_introduction_3.tex <==
\section{Introduction}
\label{sec:introduction}

%%%%%%%%%%%%%%%%%
%%% T2I models and fine-tuning of models for several downstream tasks.
%%%%%%%%%%%%%%%%%

Text-to-image (T2I) generation has recently been popularized due to the astonishing performance of state-of-the-art diffusion models such as Stable Diffusion \cite{rombach2021highresolution} and DALL·E 2 \cite{ramesh2022hierarchical}.
%
Beyond text prompt to image generation approach, variations of the T2I models have enabled a variety of fascinating applications, such as conditioned generation based on input of other modalities \cite{zhang2023adding, li2023gligen}, personalization to object instances\cite{}, and inpainting \cite{lugmayr2022repaint, Xie_2023_CVPR}.
%
Adapting T2I models to these applications generally involves fine-tuning of the models. 


%%%% Issues with fine-tuning of models.
Though fine-tuning of T2I models can adapt model to required downstream task, there are issues associated with this.
First, fine-tuning of T2I models require preparing a dataset of image-text pairs, where text is a natural language description of the corresponding image. In many cases, however, a simple text description is not enough to describe the information of an image. \VV{Give example here.}
%
Further, fine-tuning may also lead to catastrophic forgetting of the original model.
%
This is the dilemma where users have to continuously try many different text prompts via a cumbersome prompt engineering process to get the desirable generated images \cite{}.

% Moreover, when fine-tuning a T2I diffusion model, one needs to prepare 

On the other hand, prompt learning is a popular method of adapting NLP models for specific downstream tasks. 
%
Instead of giving a natural language text as prompt, a sequence of learnable embeddings serve as the prompt input of language models, and therefore improve the model performance and reduce the number of training parameter in the model itself at the same time. 
%
This method is also proven to be useful when adapted to computer vision tasks and vision-language tasks as well \cite{jia2022visual, zhou2022learning}.



In this work, we propose to adapt prompt learning approach on T2I diffusion models.
%
Specifically, when fine-tuning the diffusion model using image-text paired data, instead of using fixed text prompt and updating the weights in diffusion model itself, we insert a sequence of learnable embeddings, concatenated with the embeddings of any other meaningful words, such as the class name or object description of a set of images, as the conditioning input. 
%
These learned embeddings can be treated as a set of learned descriptions of the training images. 
%
Although they might not interpretable by human as they lie in a continuous space, the pretrained T2I diffusion model should have the ability to understand the learned embedding and generate desirable outputs.
%
Additionally, we propose a modified approach to learn a distribution of prompt instead of a fixed prompt for a set of images. This prompt distribution should be able to capture a common characteristics of the images within the same set, e.g, style, texture, pose, etc.
%
More specifically, this is done by keeping a collection of prompts corresponding to a same set of images, and the prompts are updated orthogonally so that a normal distribution could be used to model the differently updated prompts.
%
During inference, we can then sample from the prompt distribution, which should have a similar "meaning", understood by the downstream diffusion model, to produce in-distribution but at the same time diverse outputs.


The proposed approach of learning distributions over prompts can be easily adapted to several downstream T2I tasks.
% The learned prompts or distributions of prompts can be thus easily adopted to other T2I tasks. 
%
First, we demonstrate the effectivenss of our approach in customizing image generation task.
%
By taking several images of an object of interest as training images, we demonstrate that learning prompt distributions generate diverse set of images compared to the fixed prompt.
% One of the straightforward use cases would be customized image generation.
% learn a fixed prompt to generate images of similar object, or by incorporating prompt distribution learning, we can generate a more diverse set of images. 
% 
% By taking several images of an object of interest as training images, we learn a fixed prompt to generate images of similar object, or by incorporating prompt distribution learning, we can generate a more diverse set of images. 
%
Next, we show that the same approach of learning prompts can also be adapted to other existing diffusion-based pipelines that take texts as an input.
%
For example, we highlight benefits of using learned prompts for inpainting task that allows model to in-paint the masked area with a customized object. We also demonstrate effectiveness of using learned prompts for text-to-3D generation task that makes it easy to generate different customized 3D objects of same style, etc.
%
Finally, another useful case might be synthetic data generation, where we use a small dataset to learn the prompts using T2I diffusion model and then generate a larger scale in-domain dataset with enough fidelity and diversity.

\VV{We may need to refer to some figures here, also talk about some quatitative improvements over the baselines.}

\VV{Finally our key contributions are.}

==> sections/1_introduction_4.tex <==
\section{Introduction}
\label{sec:introduction}

%%%%%%%%%%%%%%%%%
%%% T2I models and fine-tuning of models for several downstream tasks.
%%%%%%%%%%%%%%%%%

Text-to-image (T2I) generation has recently been popularized due to the astonishing performance of state-of-the-art diffusion models such as Stable Diffusion \cite{rombach2021highresolution} and DALL·E 2 \cite{ramesh2022hierarchical}.
%
Beyond text prompt to image generation approach, variations of the T2I models have enabled a variety of fascinating applications, such as conditioned generation based on input of other modalities \cite{zhang2023adding,li2023gligen,yang2023reco}, inpainting \cite{lugmayr2022repaint, Xie_2023_CVPR}, image editing \cite{mokady2023null,brooks2023instructpix2pix}, and customization of instance and concept \cite{ruiz2022dreambooth,kumari2022customdiffusion}.
%
Adapting T2I models to these applications generally involves fine-tuning of the models. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Issues with fine-tuning of models.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Though fine-tuning of T2I models can adapt model to required downstream task, there are issues associated with this.
%
First, fine-tuning of T2I models requires preparing a dataset of image-text pairs, where text is a natural language description of the corresponding image, but it usually challenging to collect a diverse large scale captioned dataset.
%
% For example, to remove social bias of T2I model through fine-tuning, one needs to prepare and curate a variety of positive image-text pairs with appropriate context description, \eg, "a photo of an engineer fixing a machine in a factory", but the work is nontrivial and cumbersome through either retrieving web image data or design prompts for synthetic image generation. \brian{probably not a good example}
%
In many cases, it is also hard to prepare sufficient text description that describes the information contained in an image.
%
For example, when fine-tuning a model for different customized attributes or styles, it is often hard to describe a specific attribute or style using natural language.
%
Further, fine-tuning may also lead to catastrophic forgetting of the original model, where the original learned ability may be lost after modifying the weights for downstream tasks.
%
Failing to address these challenges will potentially result in an undesired model, and the users may need to continuously try different text prompts via a cumbersome prompt engineering process to get the desirable generated images.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Prompt tuning and limitation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
On the other hand, prompt tuning, which is a popular method of adapting NLP models for specific downstream tasks, may potentially 
%
Instead of giving a natural language text as prompt, a sequence of learnable embeddings serve as the prompt input of language models.
%
The performance on downstream tasks can be improved without tuning the pretrained model weights, and at the same time prevent catastrophic forgetting on the pretrained model. 
%
This method is also proven to be useful when adapted to computer vision tasks and vision-language tasks as well \cite{jia2022visual, zhou2022learning}.
%
However, when applied to fine-tuning of T2I model in general, it does not make sense to use one prompt to encode visual information of all images in the training set, while learning one prompt for each image would be too expensive to train. \brian{maybe change wording}
%
Thus, inspired by Lu \etal \cite{lu2022prompt}, it is natural to introduce a distribution of prompts that corresponds to a set of images. 
\brian{maybe elaborate more}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our proposed method
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this work, we propose a prompt distribution tuning approach on T2I model for various downstream tasks.
%
Specifically, when fine-tuning a T2I model using image-text paired data, instead of using fixed text prompt for each image and update the weights in T2I model itself, we use a sequence of learnable embeddings, concatenated with the embeddings of any other meaningful words, such as the class name or object description of a set of images, as the conditioning input.
%
Although they might not be interpretable by human as they lie in a continuous space, the pretrained T2I model should have the ability to understand the learned embedding and generate desirable outputs.
%
To model a distribution of prompt, instead of using one sequence as typical prompt tuning setup, we keep a set of such learnable embedding sequences to optimize orthogonally.
%
Our emphasis therefore lies in learning prompts at a category level, where a category may contain multiple object instances differ in details but share some commonalities and similar attributes, \eg a category in an image classification dataset.
%
The learned prompt distribution can be treated as a distribution of learned descriptions of the training images and should be able to capture their common attributes, e.g, style, texture, pose.
%
During inference, we can then sample from the prompt distribution, which should have a similar "meaning", understood by the downstream diffusion model, to produce in-distribution but at the same time more diverse outputs.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Use case and experiments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The proposed approach of learning distributions over prompts can be easily adapted to several downstream T2I tasks.
%
In this work, we experiment our proposed approach and demonstrate image generation using T2I diffusion model.
%
First, we demonstrate the effectiveness of our approach in customizing image generation task.
%
By taking a small set of images objects of interest as training images, we demonstrate that our approach of learning prompt distribution can generate diverse in-distribution images compared to prompt tuning method on a single fixed prompt.
%
Next, we show that the learned prompt embeddings can also be adapted to other existing diffusion-based pipelines that take texts as an input.
%
For example, we highlight capabilities of using learned prompts for text-to-3D generation task that makes it easy to generate different customized 3D objects of similar style and attributes using a small set of training images.
%
Finally, an useful case might be synthetic data generation, where we use a small dataset to learn the prompts using T2I diffusion model and then generate a larger scale in-domain dataset with enough fidelity and diversity.
\VV{We may need to refer to some figures here, also talk about some quantitative improvements over the baselines.}

In summary, our contributions are:
\begin{itemize}
    \item We propose a distribution based prompt tuning methods for learning soft prompts for T2I model.
    \item Using a public available T2I diffusion model, we experiment our approach on customization T2I generation tasks and show that our approach have the ability to generate diverse in-distribution images.
    \item Our further experiments show that our learned distribution is easy to be adapted to other generation tasks that requires text as input.
    \item We further demonstrate the effectiveness of our approach on synthetic image dataset generation tasks.
\end{itemize}

==> sections/1_introduction_5.tex <==
\section{Introduction}
\label{sec:introduction}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% T2I models and fine-tuning of models for customized generation.
%%%%%%%%%%%%%%%%%%%%%%%%%%

Text-to-image (T2I) generation has recently been popularized due to the astonishing performance of state-of-the-art diffusion models such as Stable Diffusion \cite{rombach2021highresolution} and DALL·E 2 \cite{ramesh2022hierarchical}.
%
Beyond text prompt to image generation approach, variations of the T2I models have enabled a variety of fascinating applications that allow user to provide more conditions to control the generation, such as conditioned generation based on input of other modalities \cite{zhang2023adding,li2023gligen,yang2023reco}, inpainting \cite{lugmayr2022repaint, Xie_2023_CVPR}, image editing \cite{mokady2023null,brooks2023instructpix2pix}.
%
Among the interesting applications, the idea of personalization or customization of T2I generation is popularized recently.
%
Several previous works enabled T2I model to generate novel images of personalized objects or concepts based on user provided images as reference, with the flexibility to incorporate additional natural language descriptions. 
%
This is generally done by associating a new text token with the user provided concept through fine-tuning the model parameters \cite{ruiz2022dreambooth,kumari2022customdiffusion} or newly added learnable token embeddings \cite{gal2022image}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% User may want to personalize with multiple concepts, not feasible to use natural language, and lack of diversity if using existing methods
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In many cases, however, user may want to personalize T2I generation over a more vague visual attribute instead of a specific instance or concept.
%
For example, user may want to generate a diversity of new cartoon characters with similar style or visual attributes following a set of reference images that shares some common attributes.
%
In this case, trying over multiple natural language text prompts will take lots of time and effort and hard to get desired result that follows the reference images.
%
On the other hand, using the existing methods mentioned above will result in lack of diversity, since the associated token is fixed and will typically result in an visual average of the different training images.
%
Thus, inspired by Lu \etal \cite{lu2022prompt}, it is natural to introduce a distribution of prompt tokens to associate with a set of images to capture a distribution of the common attributes expressed in the training image set. 
% \brian{maybe elaborate more}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our proposed method
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this work, we propose a prompt distribution tuning approach on T2I model for various downstream tasks.
%
Specifically, when fine-tuning a T2I model using image-text paired data, instead of using fixed text prompt for each image and update the weights in T2I model itself, we use a sequence of learnable embeddings, concatenated with the embeddings of any other meaningful words, such as the class name or object description of a set of images, as the conditioning input.
%
Although they might not be interpretable by human as they lie in a continuous space, the pretrained T2I model should have the ability to understand the learned embedding and generate desirable outputs.
%
To model a distribution of image attribute using prompts, instead of using one sequence as typical prompt tuning setup, we keep a set of such learnable embedding sequences to optimize orthogonally.
%
Our emphasis therefore lies in learning prompts at a category level, where a category may contain multiple object instances differ in details but share some commonalities and similar attributes, \eg a category in an image classification dataset.
%
The learned prompt distribution can be treated as a distribution of learned descriptions of the training images and should be able to capture their common attributes, e.g, style, texture, pose.
%
During inference, we can then sample from the prompt distribution, which should have a similar "meaning", understood by the downstream T2I model, to produce in-distribution but at the same time more diverse outputs.
%
As a result, the proposed method of prompt distribution learning on T2I model is effective in capturing distribution of visual attributes and generating customized in-distribution images.
%
Since the method is based on prompt tuning without tuning the T2I model parameters, it also prevents catastrophic forgetting of the pretrained model and at the same time parameter efficient to tune.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Use case and experiments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The proposed approach of learning distributions over prompts can be easily adapted to several downstream T2I tasks.
%
In this work, we experiment our proposed approach and demonstrate image generation using T2I diffusion model.
%
First, we demonstrate the effectiveness of our approach in customizing image generation task.
%
By taking a small set of images objects of interest as training images, we demonstrate that our approach of learning prompt distribution can generate diverse in-distribution images compared to prompt tuning method on a single fixed prompt.
%
Next, we show that the learned prompt embeddings can also be adapted to other existing diffusion-based pipelines that take texts as an input.
%
For example, we highlight capabilities of using learned prompts for text-to-3D generation task that makes it easy to generate different customized 3D objects of similar style and attributes using a small set of training images.
%
Finally, an useful case might be synthetic data generation, where we use a small dataset to learn the prompts using T2I diffusion model and then generate a larger scale in-domain dataset with enough fidelity and diversity.
\VV{We may need to refer to some figures here, also talk about some quantitative improvements over the baselines.}

In summary, our contributions are:
\begin{itemize}
    \item We propose a distribution based prompt tuning methods for learning soft prompts for T2I model.
    \item Using a public available T2I diffusion model, we experiment our approach on customization T2I generation tasks and show that our approach have the ability to generate diverse in-distribution images.
    \item Our further experiments show that our learned distribution is easy to be adapted to other generation tasks that requires text as input.
    \item We further demonstrate the effectiveness of our approach on synthetic image dataset generation tasks.
\end{itemize}




\brian{
1. different than control net, they use a very strong constraint, we guide generation on a general distribution on image level
2. reviewer may ask why don't use vae to capture image distribution
1) vae not as good as diffusion
2) no text edit flexibility
3) easier to train (efficiency, mode collapse, etc)
3. From gundam/cat experiment, if we feed images that diffusion itself is familiar with, the learned prompt may be very close to the corresponding text, and therefore can also generate diverse images
4. Training images may be not be too diverse so that pretrained diffusion have learned the general description, while too similar will not make significant difference with textual inversion with randomness in diffusion itself
}

==> sections/1_introduction_6.tex <==
\section{Introduction}
\label{sec:introduction}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% T2I models and fine-tuning of models for customized generation.
%%%%%%%%%%%%%%%%%%%%%%%%%%

Text-to-image (T2I) generation has recently been popularized due to the astonishing performance of state-of-the-art diffusion models such as Stable Diffusion \cite{rombach2021highresolution} and DALL·E 2 \cite{ramesh2022hierarchical}.
%
% Beyond text prompt to image generation approach, variations of the T2I models have enabled a variety of fascinating applications that allow user to provide more conditions to control the generation, such as conditioned generation based on input of other modalities \cite{zhang2023adding,li2023gligen,yang2023reco}, inpainting \cite{lugmayr2022repaint, Xie_2023_CVPR}, image editing \cite{mokady2023null,brooks2023instructpix2pix}.
% 
Further, variations of the T2I models have enabled several fascinating applications that allow user to control the generation, such as conditioned generation based on other input modalities \cite{zhang2023adding,li2023gligen,yang2023reco}, inpainting \cite{lugmayr2022repaint, Xie_2023_CVPR}, image editing \cite{mokady2023null,brooks2023instructpix2pix}.
%
One such interesting application is personalization of T2I models to generate novel images of objects or concepts based on user provided images as reference. 
%
Moreover, these visual concepts are also associated with new textual descriptions to provide flexibility in generation.
%
This is generally achieved by fine-tuning the model parameters \cite{ruiz2022dreambooth,kumari2022customdiffusion} or newly added learnable token embeddings \cite{gal2022image, voynov2023p+}.
%
% Among the interesting applications, the idea of personalization or customization of T2I generation is popularized recently.
%
% Several previous works enabled T2I model to generate novel images of personalized objects or concepts based on user provided images as reference, with the flexibility to incorporate additional natural language descriptions. 
%
% This is generally done by associating a new text token with the user provided concept through fine-tuning the model parameters \cite{ruiz2022dreambooth,kumari2022customdiffusion} or newly added learnable token embeddings \cite{gal2022image}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% User may want to personalize with multiple concepts, not feasible to use natural language, and lack of diversity if using existing methods
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In many cases, however, user may want to personalize T2I generation over a more vague visual attribute instead of a specific instance or concept.
%
For example, user may want to generate a diversity of new cartoon characters with similar style or visual attributes following a set of reference images that shares some common attributes.
%
In this case, trying over multiple natural language text prompts will take lots of time and effort and hard to get desired result that follows the reference images.
%
On the other hand, using the existing methods mentioned above will result in lack of diversity, since the associated token is fixed and will typically result in an visual average of the different training images.
%
Thus, inspired by Lu \etal \cite{lu2022prompt}, it is natural to introduce a distribution of prompt tokens to associate with a set of images to capture a distribution of the common attributes expressed in the training image set. \VV{We can move the previous sentence later after we propose our approach.}
% \brian{maybe elaborate more}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our proposed method
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this work, we propose a prompt distribution tuning approach on T2I model for various downstream tasks.
%
Our proposed solution has three key components. First, in order to adapt a T2I model, instead of using fixed text prompt for each image, we use a sequence of learnable embeddings and concatenate with the embeddings of any other meaningful words, such as the class name or object description of a set of images, as input to T2I model.
%
Second, to model different attributes described by reference user images using prompts, we keep a set of $K$ learnable embedding sequences to be optimized orthogonally.
%
Finally, we learn a distribution over prompt sequences that are modelled using a Gaussian mixture models.
%
% that allows us to generate diverse images for each concepts by providing diversity in prompt embedding. We use a mixture of Gaussian model to represent distribution over learnt prompt sequences. 
%

The learned prompt distribution can be treated as a distribution of learned descriptions of the user provided reference images and should be able to capture their common attributes, e.g, style, texture, pose.
%
Finally, since the method is based on prompt tuning without tuning the T2I model parameters, it also prevents catastrophic forgetting of the pretrained model and at the same time parameter efficient to tune.

During inference, we sample from the prompt distribution, which should have a similar "meaning", understood by the downstream T2I model, to produce in-distribution but at the same time more diverse outputs. 
%
As a result, the proposed method of prompt distribution learning on T2I model is effective in capturing distribution of visual attributes and generating customized in-distribution images.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Our proposed method
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In this work, we propose a prompt distribution tuning approach on T2I model for various downstream tasks.
% %
% Specifically, when fine-tuning a T2I model using image-text paired data, instead of using fixed text prompt for each image and update the weights in T2I model itself, we use a sequence of learnable embeddings, concatenated with the embeddings of any other meaningful words, such as the class name or object description of a set of images, as the conditioning input.
% %
% Although they might not be interpretable by human as they lie in a continuous space, the pretrained T2I model should have the ability to understand the learned embedding and generate desirable outputs.
% %
% To model a distribution of image attribute using prompts, instead of using one sequence as typical prompt tuning setup, we keep a set of such learnable embedding sequences to optimize orthogonally.
% %
% Our emphasis therefore lies in learning prompts at a category level, where a category may contain multiple object instances differ in details but share some commonalities and similar attributes, \eg a category in an image classification dataset.
% %
% The learned prompt distribution can be treated as a distribution of learned descriptions of the training images and should be able to capture their common attributes, e.g, style, texture, pose.
% %
% During inference, we can then sample from the prompt distribution, which should have a similar "meaning", understood by the downstream T2I model, to produce in-distribution but at the same time more diverse outputs.
% %
% As a result, the proposed method of prompt distribution learning on T2I model is effective in capturing distribution of visual attributes and generating customized in-distribution images.
% %
% Since the method is based on prompt tuning without tuning the T2I model parameters, it also prevents catastrophic forgetting of the pretrained model and at the same time parameter efficient to tune.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Use case and experiments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We evaluate the proposed approach on several generation tasks.
% 
First, we demonstrate the effectiveness of our approach in customizing image generation task.
%
By taking a small set of images of objects of interest as training images, we demonstrate that our approach generates diverse in-distribution images compared to prompt tuning method on a single fixed prompt.
%
Next, we also show that the learned prompt embeddings can also be adapted to other existing diffusion-based pipelines that take texts as an input.
%
For example, we highlight capabilities of using learned prompts for text-to-3D generation task that makes it easy to generate different customized 3D objects of similar style and attributes using a small set of training images.
%
Finally, we also show that our approach can be very effective in  generating synthetic training data generation. This is evaluated on the ImageNet dataset where we observe that the proposed approach achieves better results than prior approaches for generating synthetic training data and on-par with using real training data.
%
\VV{We may need to refer to some figures here, also talk about some quantitative improvements over the baselines.}
\VV{Some of these paragraphs are long. We can shorten them later.}

In summary, our contributions are:
\begin{itemize}
    \item We propose a distribution based prompt tuning methods for learning soft prompts for T2I model.
    \item Using a public available T2I diffusion model, we experiment our approach on customization T2I generation tasks and show that our approach have the ability to generate diverse in-distribution images.
    \item Our further experiments show that our learned distribution is easy to be adapted to other generation tasks that requires text as input.
    \item We further demonstrate the effectiveness of our approach on synthetic image dataset generation tasks.
\end{itemize}




\brian{
1. different than control net, they use a very strong constraint, we guide generation on a general distribution on image level
2. reviewer may ask why don't use vae to capture image distribution
1) vae not as good as diffusion
2) no text edit flexibility
3) easier to train (efficiency, mode collapse, etc)
3. From gundam/cat experiment, if we feed images that diffusion itself is familiar with, the learned prompt may be very close to the corresponding text, and therefore can also generate diverse images
4. Training images may be not be too diverse so that pretrained diffusion have learned the general description, while too similar will not make significant difference with textual inversion with randomness in diffusion itself
}

==> sections/4_experiments.tex <==



\section{Style/texture transfer}

\brian{
1.During training concat with label, inference use for other category, training use different scale of sketch
2. One style black\&white, others of other two colors, show that we can generate multiple color, while baseline may converge to only one.
}


\begin{itemize}
    \item Use same images in textual inversion and try output (Style/texture itself is a distribution)
    \item baseline: textual inversion, ours fixed prompt
    \item Input samples of same style images, generate e.g. street of paris, adorable corgi, in the style of input images.
    \item TODO: edit concat with prefix and suffix pre text encoder
    \item quantitative metrics: measure cosine similarity of mean and variance (No quantitative in textual inversion)
\end{itemize}

\brian{
\begin{itemize}
    \item Try same examples from textual inversion
    \item Find some diverse styles (e.g. paintings of renaissance, chinese water color, katsushika hokusai, van gogh, picasso, etc, and differnt cartoon styles, japanese anime, disney, etc.) \VV{These experiments look good.}
    \item Try some distribution learned styles with prefix/suffix texts
\end{itemize}
}






\section{Personalized 3D Object Synthesis}

\begin{itemize}
    \item TODO: try MVDream
    \item qualitative result: show comparison with dreambooth3d and mvdream using same training images
    \item qualitative result: use diverse training images, compare between fixed prompt and prompt distribution
    \item quantitative: same as personalized foreground (measure diversity)
    \VV{We should have similar experiment setup as 2D setup. What are the objects are we planning to use?}
\end{itemize}


\subsection{Ablation Studies}
\begin{itemize}
    \item n\_ctx
    \item n\_prompts
    \item n\_samples
    \item reference prompt distribution learning paper
\end{itemize}






The most straightforward experiment would be generating diverse but similar-looking images as the training images.
%
We would use a same set of training images to train ours pipeline, as well as Textual Inversion and DreamBooth as baselines, and visually compare the quality of images.
%
Since the limitation of our pipeline is that we are unable to modify the prompt using natural language to generate images of customized object in different context, for fair comparison, we would use the encoded token solely as the inference prompt in DreamBooth and Textual Inversion.


As another experiment, we will evaluate the ability of generating diverse and in-domain image data using the ImageNet-1K \citep{ILSVRC15} dataset.
%
Specifically, we will take a subset of ImageNet training set from each class as the training set, and use our pipeline to learn one fixed or one distribution of prompt for each class, and then use the learned prompt to generate a same size clone of ImageNet dataset.
%
We then evaluate the generation quality by training a ResNet-50 \citep{he2016deep} classifier using the synthetic dataset and then evaluate the classification accuracy on validation set of ImageNet. This accuracy is a metric of evaluating conditional generative models known as Classification Accuracy Score (CAS) \citep{ravuri2019classification}.
%
Due to the large scale of ImageNet dataset, we may take a subset of classes (100 classes) to perform this experiment.
%
Existing baselines include using solely class names as prompt and class names with some manual prompt engineering tricks to generate synthetic data from the pretrained Stable Diffusion pipeline \citep{sariyildiz2022fake, shipard2023boosting}. 


Other experiments: adapt learned prompt to text-to-3D diffusion models. Dreamfusion \citep{poole2022dreamfusion} is a text-to-3D generation pipeline that leverages pretrained diffusion model to generate images of different views to train a NeRF \citep{mildenhall2021nerf} without any extra 3D data.
%
By applying a learned prompt in this pipeline, we can generate customized 3D objects similar to the training images used in learning the prompts.
%
An existing baseline is DreamBooth3D \citep{raj2023dreambooth3d}, which replaces the diffusion model in DreamFusion by a customized DreamBooth diffusion to perform customized text-to-3D generation.
%

